Delaunay Ends of Constant Mean Curvature Surfaces

The generalized Weierstrass representation is used to analyze the asymptotic behavior of a constant mean curvature surface that arises locally from an ordinary differential equation with a regular singularity. We prove that a holomorphic perturbation of an ODE that represents a Delaunay surface generates a constant mean curvature surface which has a properly immersed end that is asymptotically Delaunay. Furthermore, that end is embedded if the Delaunay surface is unduloidal.

==> content-notes.tex <==
\small

\part{Notes}
\label{part3}

\section{Preliminary (notes)}

\typeout{=================notes/notation-notes.tex}
\input{notes/notation-notes.tex}
\typeout{=================notes/norm}
\input{notes/norm}
\typeout{=================notes/exp-notes}
\input{notes/exp-notes}

%------------------------------------------------
\section{Delaunay (notes)}
\typeout{=================notes/delaunay-residue-notes}
\input{notes/delaunay-residue-notes}
\typeout{=================notes/delaunay-gauge}
\input{notes/delaunay-gauge}
\typeout{=================notes/delaunay-metric}
\input{notes/delaunay-metric}
\typeout{=================notes/delaunay-frame-notes}
\input{notes/delaunay-frame-notes}
\typeout{=================notes/tau-notes}
\input{notes/tau-notes}

\typeout{=================notes/factorization-notes}
\input{notes/factorization-notes}

%-------------------------------------
\section{Growth Estimates (notes)}
\typeout{=================notes/delaunay-growth-extended-notes}
\input{notes/delaunay-growth-extended-notes}

%-------------------------------------
\section{Simple factors (notes)}
\typeout{=================notes/projection}
\input{notes/projection}

\typeout{=================notes/simplefactor-dressing-notes}
\input{notes/simplefactor-dressing-notes}

\typeout{=================notes/simplefactor-convergence-notes}
\input{notes/simplefactor-convergence-notes}


\section{Multibubbleton asymptotics: alternate (notes)}
\label{Sec:bubbleton-asymptotics-alt}
\typeout{=================notes/bubbleton-asymptotics-alt}
\input{notes/bubbleton-asymptotics-alt}

%-------------------------------------
\section{The \texorpdfstring{$z^AP$}{ZAP} lemma and gauges (notes)}
\typeout{=================notes/zap-pointwise}
\input{notes/zap-pointwise}
\typeout{=================notes/zap-notes}
\input{notes/zap-notes}
\typeout{=================notes/zap-extend}
\input{notes/zap-extend}

%--------------------------------------------
\section{Asymptotics of immersions (notes)}
\typeout{=================notes/geometry-notes}
\input{notes/geometry-notes}

\section{Expansion of the gauge equation \texorpdfstring{$\xi = \gauge{\alpha}{B}$ in $\lambda$}{xi=alpha.B in lambda} (notes)}
\typeout{=================notes/B}
\input{notes/B}


\begin{comment}
%=======================================================
%=======================================================
%=======================================================
\part{Archive material}
\label{part4}

\section{Growth Estimates (notes)}
\typeout{=================notes/delaunay-growth-notes}
\input{notes/delaunay-growth-notes}
\typeout{=================notes/delaunay-growth-near-zero}
\input{notes/delaunay-growth-near-zero}
\typeout{=================notes/delaunay-growth-near-zero-notes}
\input{notes/delaunay-growth-near-zero-notes}
\typeout{=================notes/delaunay-growth-near-S1}
\input{notes/delaunay-growth-near-S1}
\typeout{=================notes/delaunay-growth-on-S1}
\input{notes/delaunay-growth-on-S1}


\section{Asymptotics of dressed immersions (notes)}
\typeout{=================notes/bubbleton-dressing-notes}
\input{notes/bubbleton-dressing-notes}

\section{Asymptotics of Iwasawa factors (notes)}
\typeout{=================notes/iwasawa-convergence}
\input{notes/iwasawa-convergence}
\typeout{=================notes/frame-asymptotics-notes}
\input{notes/frame-asymptotics-notes}
\typeout{=================notes/keylemma}
\input{notes/keylemma}
\end{comment}


==> theorem-graph.tex <==
\begin{figure}
\includegraphics[scale=1.02, angle=90]{images/theorem-graph.pdf}
\caption{Dependency graph.}
\end{figure}

